First principles studies of the surface and opto-electronic properties of ultra-thin t-Se

Selenium is a crucial earth-abundant and non-toxic semiconductor with a wide range of applications across the semiconductor industries. Selenium has drawn attention from scientific communities for its wide range of applicability: from photovoltaics to imaging devices. Its usage as a photosensitive material largely involves the synthesis of the amorphous phase (a-Se) via various experimental techniques. However, the ground state crystalline phase of this material, known as the trigonal selenium (\textit{t}-Se), is not extensively studied for its optimum electronic and optical properties. In this work, we present density functional theory (DFT) based systematic studies on the ultra-thin $(10\overline{1}0)$ surface slabs of \textit{t}-Se. We report the surface energies, work function, electronic and optical properties as a function of number of layers for $(10\overline{1}0)$ surface slabs to access its suitability for applications as a photosensitive material.

==> a-Se Modeling/SupplementalInformation.tex <==
\section{Supplemental Material}

\vspace{10mm}
\begin{center}
\Large{First principles studies of the surface and opto-electronic properties of ultra-thin \textit{t}-Se}\\
\vspace{2mm}
\large{S. K. Barman, M. N. Huda, J. Asaadi, E. Gramellini, D. Nygren}
\end{center}

\vspace{10mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{figure}[htb]
%    \centering
%    \includegraphics[scale=0.25]{figures/FourByFourLayer.png}
%    \caption{Schematics of a (4$\times$4) (100) surface slab made of five \textit{t}-Se layers  viewed along (a) [010], (b) [100], and (c) [001] directions. This figure shows that selenium atoms on (010) and (100) planes have similar geometry while atoms on (001) plane have different geometric orientation. Hence, we present the optical properties such as absorption coefficient, reflectivity, refractive index, and electron loss function for polarizations along [100] and [001] directions. In this work, a vacuum of 25\r{A} is added on the top of each slab along [100] direction. }
%    \label{fig:4x4slab}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Surface Properties}\label{sec:Supp-SurfaceCalc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{figure}[!htbp]
%    \centering
%    \includegraphics[scale=0.25]{figures/SurfaceAreaConstrained.png}
%    \caption{GGA and GGA + vdW optimized (a) surface area (\r{A}$^2$), (b) incremental energy $\Delta$E ($eV$) at each layer, and (c) energy E$_{\text{tot}}$ (eV) of constrained \textit{t}-Se (100) surface slabs as a function of the number of layers (N). Surface areas as in (a) for constrained layers were kept fixed for GGA and GGA +vdW optimizations while (b) shows the incremental energy, $\Delta$E convergence within 0.01 $eV$. Energies for bulk selenium, $E_{bulk}$ derived from linear fitting in (c) are very close to separate bulk calculations which are within 0.001(0.023) $eV$ per unit cell for GGA(GGA + vdW) as in Table \ref{tab:TotalEnergy}.}
%    \label{fig:SurfaceAreaConstrained}
%\end{figure}


\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    & \multicolumn{2}{c|}{Surface area of free-standing laryers (\r{A}$^2$)} \\
    \hline
    Number of layers & \textbf{GGA} & \textbf{GGA + vdW} \\
    \hline
    1 & 21.08 & 20.29 \\
    \hline
    2 & 21.91 & 20.84 \\
    \hline
    3 & 22.23 & 21.08 \\
    \hline
    4 & 22.36 & 21.17 \\
    \hline
    5 & 22.44 & 21.22 \\
    \hline
    6 & 22.52 & 21.32 \\
    \hline
    7 & 22.62 & 21.35 \\
    \hline
    8 & 22.64 & 21.41 \\
    \hline
    9 & 22.61 & 21.43 \\
    \hline
    10 & 22.64 & 21.46 \\
    \hline
    11 & 22.77 & 21.46 \\
    \hline
    12 & 22.71 & 21.46 \\
    \hline
    13 & 22.68 & 21.44 \\
    \hline
    14 & 22.73 & 21.51 \\
    \hline
    15 & 22.74 & 21.53 \\
    \hline
    \end{tabular}
    \caption{GGA and GGA + vdW relaxed $(10\overline{1}0)$ surface areas of \textit{t}-Se as the number of layer increases for free standing layers.}
    \label{tab:SurfaceAreas}
\end{table}



\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    & \multicolumn{2}{c|}{Surface energies, $\gamma\text{(mJ/m}^2$) for $(10\overline{1}0)$ surface slabs of \textit{t}-Se} \\
    \hline
 %   & \multicolumn{2}{|c}{\textbf{Free standing layers}} & \multicolumn{2}{|c|}{\textbf{Constrained layers}} \\
 %   \hline
    Number of layers in slabs & GGA & GGA \\ %+ vdW & GGA & GGA + vdW \\
    \hline
    1 & 160.22 & 176.24 \\ %& 160.30 & 160.30 \\
    \hline
    2 & 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    3 & 160.22 & 192.26 \\%& 160.30 & 192.30 \\
    \hline
    4 & 160.22 & 192.26 \\%& 160.30 & 192.30 \\
    \hline
    5 & 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    6 & 160.22 & 192.26 \\%& 160.30 & 192.30 \\
    \hline
    7 & 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    8 & 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    9 & 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    10& 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    11& 160.22 & 192.26 \\%& 160.30 & 176.30 \\
    \hline
    12& 160.22 & 176.24 \\%& 160.30 & 176.30 \\
    \hline
    13& 160.22 & 176.24 \\%& 160.30 & 176.30 \\
    \hline
    14& 160.22 & 176.24 \\%& 160.30 & 176.30 \\
    \hline
    15& 160.22 & 176.24 \\%& 160.30 & 176.30 \\
    \hline
    \end{tabular}
    \caption{GGA and GGA + vdW calculated energies of fully relaxed $(10\overline{1}0)$ surface slabs as a function of the number of layers. Atoms in this relaxation (free-standing layers) could relax in all three directions inside the simulation box.}%, whereas atoms in the constrained layers could relax along [100] (vacuum) direction only.}
    \label{tab:TotalEnergyByLayer}
\end{table}



\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    &\multicolumn{2}{c|}{Slab Thickness (\r{A})} \\
    \hline
%    & \multicolumn{2}{|c}{\textbf{Free standing layers}} & \multicolumn{2}{|c|}{\textbf{Constrained layers}} \\
%    \hline
    Number of layers in slabs & GGA & GGA + vdW \\%& GGA & GGA + vdW \\
    \hline
    2 & 4.583 & 4.283 \\%& 4.467 & 4.220 \\
    \hline
    3 & 9.056 & 8.531 \\%& 8.988 & 8.428 \\
    \hline
    4 & 14.592 & 12.690 \\%& 13.515 & 12.641 \\
    \hline
    5 & 18.065 & 16.903 \\%& 18.008 & 16.893 \\
    \hline
    6 & 22.628 & 21.123 \\%& 22.540 & 21.041 \\
    \hline
    7 & 27.150 & 29.614 \\%& 27.029 & 25.248 \\
    \hline
    8 & 31.568 & 29.614 \\%& 31.537 & 29.610 \\
    \hline
    9 & 36.109 & 33.788 \\%& 36.009 & 33.756 \\
    \hline
    10& 40.604 & 38.081 \\%& 40.464 & 38.022 \\
    \hline
    11& 45.087 & 42.232 \\%& 45.014 & 42.223 \\
    \hline
    12& 49.604 & 46.427 \\%& 49.539 & 46.513 \\
    \hline
    13& 54.102 & 50.576 \\%& 54.012 & 50.707 \\
    \hline
    14& 58.617 & 54.919 \\%& 58.562 & 54.977 \\
    \hline
    15& 63.045 & 59.217 \\%& 63.004 & 59.375 \\
    \hline
    \end{tabular}
    \caption{GGA and GGA + vdW optimized slab thickness as a function of the number of layers.}
    \label{tab:LayerThickness}
\end{table}


\FloatBarrier
\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bulk Electronic Properties}\label{sec:Supp-Bulk-Elec-Prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.4]{figures/BandStructure-Bulk.png}
    \caption{(a) GGA and (b) GGA + vdW calculated band structures of pure bulk \textit{t}-Se. The calculated indirect(direct) band gaps are 0.98(1.21) $eV$ and 0.72(0.80) $eV$, respectively. The Fermi level, $E_F$ is set at 0 $eV$. van der Waals correction, vdW was applied through the zero damping DFT-D3 method of Grimme.}
    \label{fig:BandStructure-Bulk}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.6]{figures/DOS-Bulk.png}
    \caption{GGA and GGA + vdW calculated the density of states (DOS) of pure bulk \textit{t}-Se. This figure shows that the top of the valence band and the bottom of the conduction band are mainly composed of Se $p$. Hence, the bands in Figure \ref{fig:BandStructure-Bulk} in the energy range of (-4, 4) are contributed primarily by Se $p$. The Fermi level, $E_F$ in this figure is set at 0 $eV$.}
    \label{fig:DOS-Bulk}
\end{figure}

\FloatBarrier

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Electron Density}\label{sec:Supp-Elec-Density}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htb]
 %   \centering
  %  \includegraphics[scale=0.30]{figures/ElectronDensity-Layers.png}
   % \caption{ Electron density around selenium atoms (at same isosurface level) in free-standing and constrained layers optimized and calculated through GGA + vdW. The figure shows that at the same isosurface level there is no  electron density overlap between layers in constrained slabs.}
    %\label{fig:Elec-Density}
%\end{figure}

%\FloatBarrier






\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Constrained Optical Properties}\label{sec:Supp-Con-Optical-Prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[htb]
%    \centering
%    \includegraphics[scale=0.25]{figures/OpticalProp-GGA-Constrained.png}
%    \caption{GGA calculated optical properties as a function of photon energy for constrained \textit{t}-Se (100) surface slabs having up to fifteen atomic layers. Optical properties are calculated along [100] (left panel) and [001] (right panel) directions.}
%    \label{fig:OpticalProp-GGA-SurfaceConstrained}
%\end{figure}

%\begin{figure}[htb]
 %   \centering
  %  \includegraphics[scale=0.25]{figures/OpticalProp-GGA+vdW-Constrained.png}
  %  \caption{GGA + vdW calculated optical properties as a function of photon energy for constrained \textit{t}-Se (100) surface slabs having up to fifteen atomic layers. Optical properties are calculated along [100] (left panel) and [001] (right panel) directions.}
 %   \label{fig:OpticalProp-GGA+vdW-SurfaceConstrained}
%\end{figure}
